UniWav: Towards Unified Pre-training for Speech Representation Learning and Generation

Pre-training and representation learning have been playing an increasingly important role in modern speech processing. Nevertheless, different applications have been relying on different foundation models, since predominant pre-training techniques are either designed for discriminative tasks or generative tasks. In this work, we make the first attempt at building a unified pre-training framework for both types of tasks in speech. We show that with the appropriate design choices for pre-training, one can jointly learn a representation encoder and generative audio decoder that can be applied to both types of tasks. We propose UniWav, an encoder-decoder framework designed to unify pre-training representation learning and generative tasks. On speech recognition, text-to-speech, and speech tokenization, UniWav achieves comparable performance to different existing foundation models, each trained on a specific task. Our findings suggest that a single general-purpose foundation model for speech can be built to replace different foundation models, reducing the overhead and cost of pre-training.

==> figures/spec_nfe.tex <==
\begin{figure*}[h]
\begin{center}
\centerline{\includegraphics[width=\linewidth]{spec_nfe.png}}
\end{center}
\vspace{-20pt}
\caption{ Utterence {\small \texttt{7176-88083-0014}} from {\small \texttt{test-clean}}
}
\vspace{-10pt}
\end{figure*}

==> related_work.tex <==
The success of self-supervised representation learning has emerged as a promising direction for enhancing model generalization, leading to general-purpose speech and audio intelligent systems. In recent years, the research community has witnessed significant advancements in self-supervised learning techniques across speech and other domains, with notable developments ranging from VQ-VAE \cite{van2017neural,dhariwal2020jukebox} to Data2Vec \cite{baevski2022data2vec}, among many others \cite{schneider2019wav2vec,baevski2020wav2vec2}.

Our work contributes to this growing body of research by focusing on learning quantized codebooks and rethinking the potential of jointly modeling both speech understanding and generation, aiming for a unified framework that can seamlessly integrate these tasks.

We would also like to acknowledge several previous efforts in this space and highlight potential avenues for future research, particularly in bridging the gap between speech representation learning and generative modeling.


% The success of self-supervised representation learning as one promising direction to boost model generalization for robust speech and audio understanding. In recent years, our research community has witnessed the development of many self-supervised learning methods for speech and other domains, from VQ-VAE \cite{van2017neural,dhariwal2020jukebox} to Data2Vec \cite{baevski2022data2vec} and many others \cite{schneider2019wav2vec,baevski2020wav2vec2}. 




%Despite their ability to learn compact speech representations, we argue that there can be mismatch between the properties of the learned representation and desirable properties for speech synthesis. For example, a speech representation learned with an objective function based on minimizing reconstruction loss in euclidean space could map phonemes with small euclidean distance such as /b/ and /p/ to the same code,  while using multiple codes to replicate different types of room noise given their large euclidean distance.



%In addition, we argue that such representations have entangled salient speech attributes, thus making it hard to independently control or to model speech attributes individually. In fact, several speech synthesis frameworks \cite{siuzdak2022wavthruvec,choi2021neural} reported having to carefully chose which Wav2Vec \cite{schneider2019wav2vec} hidden layer to use such that different attributes are less entangled and can be controlled independently.

%In addition, although it is common practice \cite{siuzdak2022wavthruvec, choi2021neural} to use codes that entangle information about speech factors attributes, we observe that this entanglement can make optimization harder and limit the codes usability in tasks where disentanglement is a requirement, such as timbre conversion, language transfer and zero-shot text to speech synthesis.
	
Concurrent with the development of self-supervised learning methods for speech representation learning, the voice conversion community has made large strides in obtaining factorized speech representations, from AutoVC \cite{qian2019autovc} to \cite{nguyen2022nvc} and many others \cite{kashkin2022hifi,qian2020unsupervised,merritt2022text}. While some approaches rely on hidden representations obtained from speech to text models (S2T, ASR) \cite{kashkin2022hifi,nguyen2022nvc,merritt2022text}, other approaches rely on jointly learned speech attribute encoders and data augmentation to disentangle speech attributes \cite{qian2019autovc,qian2020unsupervised}. Our work is closest to methods that learn encoders \cite{qian2020unsupervised,merritt2022text,choi2021neural} that attempt to disentangle speech attributes. However, rather than relying on large scale unsupervised pretraining, our method leverages domain knowledge, careful data augmentation, and a set of losses to produce a vector quantized speech representation that generalizes well to unseen data, is robust to degraded audio and, above all, produces a disentangled representation of speech attributes. 

%Undoubtedly, the objective function used for S2T models is more aligned with learning a disentangled speech representation that focuses on phonemes and is invariant to  speaker timbre, acoustic conditions and such. However, S2T models are trained such that a word pronounced in different ways, due to a speaker's accent, maps to the same sequence of tokens, thus arguably collapsing a multi-modal distribution. 

%In speech synthesis it is more important to be able to clearly
%distinguish between phonemes that are close in euclidean
%space, like /p/ and /b/ for example, than to distinguish
%between non-speech sounds that are distant in euclidean
%space. Hence, a na\"ive self-supervised baseline can suffer
%from a mismatch between its objectve function used to learn
%the speech representation and the requirements of our task.
%Hence, we leverage domain knowledge and text labels to
%regularize the solution space of the representation learning
%algorithm to promote these requirements.

%For example, \fzero invariance is obtained by using some \fzero modification tool to modify F0 and minimize the distance between the hidden representation of all F0 augmented samples. 

%Unlike other approaches that assume that a single timbre vector should be used for a single speaker and that argue that one should minimize the distance between speaker encoder posterior samples from the same speaker, we argue that this would not be necessary given that the variance would anyway be stored in the residual and sampled during inference. Instead, we use a VAE formulation to leverage the disentanglement and generalization benefits it brings.

\paragraph{Speech Synthesis }

(to-be-revised) Finally, with the exception of speech synthesis models like \cite{kim2021guided,kim2022guided,valle2020flowtron,shih2022generative} that support out-of-domain adaptation through guidance or posterior sampling, most speech synthesis models are deterministic or gan-based, hence not supporting posterior sampling nor guidance.

==> tables/tokenize_full.tex <==
\begin{table*}[t!]
    \centering
    \caption{
    % \small
       Speech tokenization and resynthesis results.
       All models are trained on LibriSpeech and have a frame rate of 50Hz.
       Methods sharing the same bitrate are highlighted with the same color.
       Visualized audio samples are provided in \S\Cref{sec:spec} and audible samples are available on  \href{https://uniwav-demo.github.io/}{\texttt{\footnotesize{demo page}}}.
    }
    \label{tab:tok}
    % \vspace{3pt}
    \resizebox{\linewidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{lccHccHccHccHcc}
        \toprule
        & \multirow{2}{*}{quantization} & \multirow{2}{*}{bitrate} & & \multicolumn{2}{c}{ASR-WER$\downarrow$}& & \multicolumn{2}{c}{UTMOS$\uparrow$} & & \multicolumn{2}{c}{Spkr. Sim.$\uparrow$} & & \multicolumn{2}{c}{ViSQOL$\uparrow$} \\
        \cmidrule{4-6}
        \cmidrule{8-9}
        \cmidrule{11-12}
        \cmidrule{14-15}
        & & & &  dev & test & &  dev & test & &  dev & test  & &  dev & test \\
        \midrule
        \midrule
        Ground Truth & - & 256k & & 3.2 & 3.4 & & 3.87 & 3.77 & & - & - & & - & -  \\
        \midrule
        \rowcolor{cyan!10}
        \cellcolor{white}\multirow{3}{*}{Encodec \textsuperscript{a}} & $\text{VQ}_{1024}$ & 500 & & 41.7 & 41.0 & &  1.24 & 1.24 & & 0.25 & 0.25 & & 2.96 & 2.88 \\
        &\cellcolor{pink!20} $\text{RVQ}_{2\times1024}$& \cellcolor{pink!20}1k & & \cellcolor{pink!20}9.6 & \cellcolor{pink!20}10.3 & &  \cellcolor{pink!20}1.52 & \cellcolor{pink!20}1.50 & & \cellcolor{pink!20}0.60 & \cellcolor{pink!20}0.60& & \cellcolor{pink!20}3.59 & \cellcolor{pink!20}3.47 \\
        & $\text{RVQ}_{8\times1024}$& 4k & & 3.8 & 4.0 & & 2.94 & 2.82 & & 0.89 & 0.89 & & 4.25& 4.21 \\ 
        \midrule
        \rowcolor{cyan!10}
        \cellcolor{white}\multirow{3}{*}{DAC \textsuperscript{b}} & $\text{VQ}_{1024}$ & 500 & & 80.9 & 80.6 & &  1.24 & 1.24 & & 0.11 & 0.10 & & 1.88 & 1.73 \\
        &\cellcolor{pink!20} $\text{RVQ}_{2\times1024}$& \cellcolor{pink!20}1k & & \cellcolor{pink!20}22.8 & \cellcolor{pink!20}24.2 & &  \cellcolor{pink!20}1.28 & \cellcolor{pink!20}1.28 & & \cellcolor{pink!20}0.33 & \cellcolor{pink!20}0.31 & & \cellcolor{pink!20}2.95 & \cellcolor{pink!20}2.70 \\
        & $\text{RVQ}_{8\times1024}$& 4k & & 3.8 & 4.1 & & 3.09 & 3.03 & & 0.87 & 0.87 & & 4.42 & 4.39\\ 
        \midrule
        \rowcolor{cyan!10}
        \cellcolor{white}$\text{HuBERT}_\textsc{Base}$ \textsuperscript{c} & $\text{KM}_{1024}$ & 500 & & 9.8 & 10.2 & &  2.36 & 2.37 & & 0.14 & 0.15 & & 2.14 & 2.15 \\
        $\text{HuBERT}_\textsc{Large}$\textsuperscript{c} &\cellcolor{cyan!10} $\text{KM}_{1024}$ &\cellcolor{cyan!10} 500 & &\cellcolor{cyan!10} 7.6 &\cellcolor{cyan!10} 7.9 & &\cellcolor{cyan!10}  2.66 &\cellcolor{cyan!10} 2.65 & &\cellcolor{cyan!10} 0.14 &\cellcolor{cyan!10} 0.15 & &\cellcolor{cyan!10} 2.00 &\cellcolor{cyan!10} 2.03 \\
        \midrule
        \rowcolor{cyan!10}
        \cellcolor{white}\multirow{3}{*}{SpeechTokenizer\textsuperscript{d}} & $\text{VQ}_{1024}$ & 500 & & 10.5 & 11.0 & &  1.25 & 1.26 & & 0.16 & 0.16 & & 1.97 & 2.03 \\
        &\cellcolor{pink!20} $\text{RVQ}_{2\times1024}$& \cellcolor{pink!20}1k & & \cellcolor{pink!20}8.5 & \cellcolor{pink!20}9.1 & &  \cellcolor{pink!20}2.20 & \cellcolor{pink!20}2.08 & & \cellcolor{pink!20}0.34 & \cellcolor{pink!20}0.34 & &\cellcolor{pink!20}3.04 & \cellcolor{pink!20} 3.03 \\
        & $\text{RVQ}_{8\times1024}$& 4k & & 4.5 & 4.9 & &  3.65 & 3.56 & & 0.83 & 0.83 & & 4.22 & 4.20 \\
        \midrule
        \rowcolor{cyan!10}
        \cellcolor{white}\multirow{2}{*}{\proposed} &  $\text{KM}_{1024}$ & 500 & & 7.2 & 7.1 & &  3.64 & 3.59 & & 0.25 & 0.26 & & 2.14 & 2.09 \\
        &\cellcolor{pink!20} $\text{KM}_{2\times1024}$\textsuperscript{e} &\cellcolor{pink!20}1k & &\cellcolor{pink!20}5.6 & \cellcolor{pink!20}5.6 & & \cellcolor{pink!20}3.79 &\cellcolor{pink!20}3.72 & &\cellcolor{pink!20}0.49 &\cellcolor{pink!20}0.50 & & \cellcolor{pink!20}2.96 &\cellcolor{pink!20}2.92 \\
        \bottomrule
    \end{tabular}
    \begin{tablenotes}[flushleft]
        \item{~}{\footnotesize $\textsuperscript{a}$\citet{Defossez2022HighFN}; $\textsuperscript{b}$\citet{kumar2024high}; $\textsuperscript{c}$ with unit-HifiGAN \citet{polyak2021speech,nguyen2023expresso};    $\textsuperscript{d}$\citet{zhang2023speechtokenizer};
        $\textsuperscript{e}$ Residual quantization, see Eq.(\ref{eq:rvq})}\\
    \end{tablenotes}
    \end{threeparttable}
    }
\vspace{-5pt}
\end{table*}
